DuInNet: Dual-Modality Feature Interaction for Point Cloud Completion

To further promote the development of multimodal point cloud completion, we contribute a large-scale multimodal point cloud completion benchmark ModelNet-MPC with richer shape categories and more diverse test data, which contains nearly 400,000 pairs of high-quality point clouds and rendered images of 40 categories. Besides the fully supervised point cloud completion task, two additional tasks including denoising completion and zero-shot learning completion are proposed in ModelNet-MPC, to simulate real-world scenarios and verify the robustness to noise and the transfer ability across categories of current methods. Meanwhile, considering that existing multimodal completion pipelines usually adopt a unidirectional fusion mechanism and ignore the shape prior contained in the image modality, we propose a Dual-Modality Feature Interaction Network (DuInNet) in this paper. DuInNet iteratively interacts features between point clouds and images to learn both geometric and texture characteristics of shapes with the dual feature interactor. To adapt to specific tasks such as fully supervised, denoising, and zero-shot learning point cloud completions, an adaptive point generator is proposed to generate complete point clouds in blocks with different weights for these two modalities. Extensive experiments on the ShapeNet-ViPC and ModelNet-MPC benchmarks demonstrate that DuInNet exhibits superiority, robustness and transfer ability in all completion tasks over state-of-the-art methods. The code and dataset will be available soon.

==> sec/7_IEEEbiography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/XinpuLiu.jpg}}]{Xinpu Liu} received the B.E. degree in communication engineering and the M.E. degree in information and communication engineering from the National University of Defense Technology (NUDT), Changsha 410000, China, in 2020 and 2022, respectively, where he is currently pursuing the Ph.D. degree with the College of Electronic Science and Technology in NUDT. His research interests focus on 3D Computer Vision, particularly on point cloud completion and object detection. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/BaolinHou.jpg}}]{Baolin Hou} received the B.E. degree in electronic engineering and the M.E. degree in electronic information from the National University of Defense Technology (NUDT), Changsha 410000, China, in 2015 and 2023, respectively. His research interests focus on 3D scene and point cloud completion. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/HanyunWang.jpg}}]{Hanyun Wang} is currently an associate professor at the School of Surveying and Mapping, Information Engineering University, China. He received his Ph.D. degree from National University of Defense Technology in 2015. He was a visiting Ph.D. student at Xiamen University from 2011 to 2014. He has authored over 50 articles in journals and conferences, such as IEEE TPAMI, IEEE TGRS, ISPRS Journal P\&RS, and CVPR. His current research interests focus on 3D computer vision, remote sensing image understanding, and artificial intelligence. He also served as the guest editor for the IET Computer Vision and the managing guest editor for the International Journal of Applied Earth Observation and Geoinformation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/KeXu.jpg}}]{Ke Xu} received the M.S. and Ph.D. degrees in information and communication engineering from the National University of Defense Technology (NUDT), Changsha 410000, China, in 2006 and 2011, respectively. From 2008 to 2009, he was a visiting Ph.D. student with the University of Windsor, Windsor, ON, Canada. He is currently an Associate Professor with the College of Electronic Science and Technology in NUDT. His current research interests include intelligent information processing, underwater acoustic signal processing, and digital signal processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/JianweiWan.jpg}}]{Jianwei Wan} received the Ph.D. degree in signal and information processing from the National University of Defense Technology (NUDT), Changsha 410000, China, in 1999. He was a Senior Visiting Scholar with the University of Windsor, Windsor, ON, Canada, from 2008 to 2009. He is currently a Professor with the College of Electronic Science and Technology in NUDT. He has authored more than 100 journal and conference publications. His current research interests include signal processing, remote sensing, computer vision, pattern recognition, and hyperspectral image processing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/YulanGuo.jpg}}]{Yulan Guo} (Senior Member, IEEE) received the B.E. and Ph.D. degrees from National University of Defense Technology (NUDT) in 2008 and 2015, respectively. He has authored over 100 articles at highly referred journals and conferences. His current research interests focus on 3D vision, particularly on 3D feature learning, 3D modeling, 3D object recognition, and scene understanding. He served as an associate editor for IEEE Transactions on Image Processing, IET Computer Vision, IET Image Processing, and Computers \& Graphics. He also served as an area chair for CVPR 2023, CVPR 2021, ICCV 2021, and ACM Multimedia 2021. He organized several tutorials, workshops, and challenges in prestigious conferences, such as CVPR 2016, CVPR 2019, ICCV 2021, 3DV 2021, CVPR 2022, ICPR 2022, ECCV 2022, CVPR 2023 and CVPR 2024. He is a Senior Member of ACM.
\end{IEEEbiography}
